The Pseudo-Reachability Problem for Diagonalisable Linear Dynamical Systems

We study fundamental reachability problems on pseudo-orbits of linear dynamical systems. Pseudo-orbits can be viewed as a model of computation with limited precision and pseudo-reachability can be thought of as a robust version of classical reachability. Using an approach based on $o$-minimality of $\reals_{\exp}$ we prove decidability of the discrete-time pseudo-reachability problem with arbitrary semialgebraic targets for diagonalisable linear dynamical systems. We also show that our method can be used to reduce the continuous-time pseudo-reachability problem to the (classical) time-bounded reachability problem, which is known to be conditionally decidable.

==> discrete-setup.tex <==
% !TEX root = main.tex
\section{The discrete-time pseudo-reachability problem}
\label{sec::dis-pseudo-reach}
\TK{I dump it here...} In the following sections we prove the decidability of the pseudo-reachability problem for (discrete and continuous) diagonalisable \emph{affine dynamical systems}, which are a generalisation of LDS. 
The reason is that the classical reachability problem for affine dynamical systems can be reduced to the reachability problem for LDS by a well-known homogenisation trick (i.e. increasing the dimension by one and adding a coordinate that is kept at a constant value). For problems where control inputs (even arbitrarily small at each step) are allowed, however, this reduction does not work and affine systems require specialised treatment. 

Let $M \in \rats^{d \times d}$ be an update matrix, $s \in \rats^d$ a starting point, $b \in \rats^d$ an affine term and $S \subseteq \reals^d$ a semialgebraic target set. A sequence $x_0 = s, x_1, \ldots$ is an \emph{$\epsilon$}-pseudo-orbit of $s$ under $M$ if $||Mx_n + b - x_{n+1}||_\infty <\epsilon$ (that is, $Mx_n +b - x_{n+1} \in [-\epsilon,\epsilon]^d$) for all $n$. 

The pseudo-reachability problem asks to determine (given $M, b, s$ and $S$), whether for each $\epsilon>0$ there exists an $\epsilon$-pseudo-orbit of $s$ under the dynamics $x_{n+1}=Mx_n+b$ that reaches the set $S$. 
We now derive an equivalent formulation of the problem in terms of control sets (in the sense of linear controlled systems) that we will use for the rest of the paper.

\begin{proposition}[The control perspective]
	\label{convenient-control-set}
	Consider a compact set $\B \subseteq \reals^d$ which contains an origin-centered ball. Then the pseudo-reachability problem defined above is equivalent to the following problem:
	Given a start point $s$ and dynamics , where $u_n$ is an element of the control set $\epsilon\B $, does there exist a control sequence reaching $S$ for every $\epsilon$?
\end{proposition}
\begin{proof}
	Observe that the \emph{$\epsilon$}-pseudo-orbit dynamics can be considered as $x_{n+1}=Mx_n+b + u_n$, where $u_n$ is an element of the control set $\epsilon[-1,1]^d$, ie, the unit hypercube scaled by $\epsilon$. However, the pseudo-reachability problem asks for reachability for all $\epsilon$, and thus it does not really matter what shape the control set  $\B$ is, as long as there exist non-zero constants $C_1$ and $C_2$ such that $C_1[-1,1]^d \subseteq \B \subseteq C_2[-1,1]^d$.
	Given any control sequence for a set $\epsilon_1\B$ there exists $\epsilon_2$ such that the sequence is a valid control sequence for a set $\epsilon_2[-1,1]^d$ and vice versa. Thus the problems are equivalent.
	
	Note that this would not work if $\epsilon$ was fixed as part of the input, which we call the $\epsilon$-pseudo-reachability problem (discussed in Section \ref{hardness}).
\end{proof}

%Can choose the shape of the control set. 
%%The problem is Turing-equivalent to deciding whether for all $\epsilon>0$, there exists $n$ such that $\PO_\epsilon(n)$ intersect $S$.
%We choose the following ``product of $\ell_2$-balls'' as our control set. \JD{advantage of this is that rotations can be folded in}
%\[
%\B = \Pi_{i=1}^k B((0,0),1) \times \Pi_{i=k+1}^{d}[-1,1].
%\]
Observe that multiplying the control set by an invertible change of basis matrix satisfies the conditions of Proposition $\ref{convenient-control-set}$. Thus we have a useful corollary:

\begin{corollary}
	\label{discrete-jordan-translation}
	We may assume that the matrix $M$ is in real Jordan form.
\end{corollary}


\subsection{A closed form for the time-bounded $\epsilon$-pseudo-orbit in case $M$ is diagonalisable}
Let us denote by $\PO_\epsilon(n)$ the set of all points that are $\epsilon$-pseudo-reachable at exactly time $n$. The pseudo-reachability problem is equivalent to determining whether for all $\epsilon>0$ there exists $n$ such that $\PO_\epsilon(n)$ intersects $S$.

Write $M = D R$ where $D = \operatorname{diag}(\rho_1, \rho_1, \ldots, \rho_k, \rho_k, \rho_{k+1}, \rho_{k+2}, \ldots, \rho_{d})$ is diagonal with $\rho_i = \rho(\Lambda_i)$ for $1 \leq i \leq k$ and $R$ is a block-diagonal matrix that consists of blocks that are either $2\times2$ rotation matrices or have dimension $1\times 1$.
We fix a corresponding `rotation-invariant' control set \[
\B = \Pi_{i=1}^k B((0,0),1) \times \Pi_{i=k+1}^{d}[-1,1],
\]where $B((0,0),1)$ is the standard unit disc.

Summing the dynamics $x_{n+1}=Mx_n+b + u_n$, observe that $\PO_\epsilon(n) = M^ns + \sum_{i=0}^{n-1}M^ib + \epsilon \sum_{i=0}^{n-1}M^i\B$. Since (we chose $\B$ such that) $R\B = \B$, we have
\[
\PO_\epsilon(n)= D^n R^n s + \sum_{i=0}^{n-1}M^ib + \epsilon\sum_{i=1}^{n-1} D^iR^i\B = D^n R^n s + \sum_{i=0}^{n-1}M^ib + \epsilon \B(n)
\]
where $\B(n) = \sum_{i=1}^{n-1} D^i\B$. Observe that 
\[
\B(n) = \Pi_{i=0}^k B\left((0,0), \sum_{m=0}^{n-1} \rho_i^m\right) \times 
\Pi_{i=k+1}^d B\left(0, \sum_{m=0}^{n-1} \rho_i^m\right).
\] 
Since $\sum_{d=0}^{n-1} \rho_i^m$ is either $\frac{\rho_i^n-1}{\rho_i-1}$ or $n \rho_i$, we can write
$\B(n) = \{x : \varphi(x,n, \rho_1^n, \ldots, \rho_d^n)\}$, where $\varphi$ is a semialgebraic function.

We can apply the same case-wise summation technique to the affine term $\sum_{i=0}^{n-1}M^ib$ to get a closed form $\sum_{i=0}^{n-1}M^ib  = D^nR^nx' + cn + d$, where $x'$, $c$ and $d$ are fixed vectors. We fold $s$ and $x'$ into $x$ to get the final closed form \[
\PO_\epsilon(n)= D^n R^n x + cn +d + \epsilon \B(n).
\]

%\JD{This might be a good place to write an overview of the argument: something along the lines of , for diagonalizable M we can write an abstraction of $\PO_\epsilon(n)$ in first order logic and then use quantifier elimination }

%We can write $ \sum_{i=0}^{n-1}M^ib$ as $M^ns' +cn + d$, where $c$ and $d$ are constant vectors. Here $M^ns'$ and $d$ come from a geometric summation over eigenvalues\JD{to be explained clearly}Thus the pseudo-reachability problem is to determine, whether for all $\epsilon>0$ there exists $n$ such that $\PO_\epsilon(n)=M^nx + cn + d + \epsilon \sum_{i=0}^{n-1}M^i\B$ intersects $S$.

==> questions.tex <==
% !TEX root = main.tex
\section{non-diagonalisable decidability}
	We first notice that it's enough to consider the following \emph{accumulated} control sets to answer the pseudo-reachability problem for defining $\PO_\epsilon(n)$:
	$$\B_i(n)=\begin{cases}B\quad\rho_i<1\\\M_i^{n}B\quad\rho_i> 1\\
		\sum_{j=0}^{n-1}M_i^jB\quad\rho_i=1\end{cases},$$
	\begin{comment}
	Let $v(n)=\sum_{i=0}^{n-1}M^ib$. We modify the definition of $\PO_\epsilon(n)$ by using the above control sets and $\PO_\epsilon(n)= M^n x + v(n)+ \epsilon \B(n)$. Let the \emph{normalised} $\epsilon$-pseudo-orbit at time $n\in\nats$ to be defined as follows:
	$$\PO^{norm}_{\epsilon,i}(n)=\begin{cases}\PO_{\epsilon,i}(n)-v_i(n)\quad\rho_i\leq 1\\(\PO_{\epsilon,i}(n)-v_i(n))/\rho_i^n\quad\rho_i> 1\end{cases},$$
	for $1\leq i \leq d$.
	Also, we can define the \emph{projected time-varying surrogate corresponding to the target set} at time $n$ in the following sense: in every polynomial, all instances of state variables $y_i(n)$ whose corresponding block's spectral radius is larger than $1$ (i.e., $\rho_i>1$) is replaced by $\rho_i^ny_i(n)+v_i(n)$ and for the rest of blocks (i.e., when $\rho_i\leq 1$) we replace $y_i(n)$ with $y_i(n)+v_i(n)$. Then, we have
	$$\PO_{\epsilon}(n)\cap S\neq \emptyset\Leftrightarrow \PO_{\epsilon}^{norm}(n)\cap S^{Proj}\neq \emptyset$$
	
	(The above formulation of $S^{proj}$ isn't accurate and is just meant to compensate for the effect of normalisation applied to the pseudo-orbit.)
	
	\end{comment}
	We may notice that for the non-diagonalisable matrices $M$, the above definition of $\B(n)$ does not give us a closed form and hence prevents us from answering the pseudo-reachability problem as we cannot encode it in the required FO fashion. For this reason, we look for simpler (over-approximating) abstractions which yet are useful. %Let $\T$ to be defined in the same sense as defined for the robust reachability problem ($\T = \operatorname{cl}(\{(\gamma_1^n,\ldots, \gamma_k^n) : n \in \nats\})$). Let $\T_i$ to be the abstraction corresponding to the $i^{th}$ block. 
	We define $\B^o_\epsilon$ as follows: $$\B^{o}_{i}(n)=\begin{cases}B\quad\rho_i\neq1\\\M_i^{n-1}B\quad\rho_i> 1\\
		%\sum_{j=0}^{n-1}\T_i^jB
		\Pi_{k=1}^{\sigma_i}[l_k^o(n),u_k^o(n)]\quad\rho_i=1\end{cases},$$
	where $B$ denotes product of $\sigma_i$  appropriately sized balls (2-d for complex and 1-d for real blocks), and $[l_k^o(n), u_k^o(n)]$ denotes the (over-approximate) interval containing the projection of $\B_i(n)$ onto the $k^{th}$ coordinate. Intuitively, for blocks with $\rho<1$ and $\rho>1$, we consider perturbations only at the end and at the beginning, respectively. %Also, note that the control set over the unstable blocks is normalised (otherwise, it should have been multiplied by $D_i^{n-1}$). 
	Only, for blocks whose eigen value is of modulus one, we take the full control set into account. 
	%For the blocks with $\rho_i=1$, we define $\B_i^A(n)=\Pi_{k=1}^{\sigma_i}[l_k,u_k]$, where $[l_k, u_k]$ denotes the interval containing the projection of $\B^{norm}_i(n)$ into the $k^{th}$ coordinate. 
	For the blocks with $\rho=1$, we have $\B_i(n)\subseteq \B_i^A(n)$ for every $n\in\nats$. %For the blocks with $\rho>1$, we define $\B_i^A(n)=\T_i^{n-1}B$.
	For the blocks with $\rho>1$, we have that $\rho_i^{n'}\B_i^A(n)=\B_i(n')$ for every $n'\geq n$. Finally, for the blocks with $\rho_i< 1$, we have $ \B_i^A(n')=\B_i(n)$ for every $n'\geq n$. Note that we can compute a closed-form for $\B^A(n)$. We have the following lemma.
	\begin{lemma}\label{lem:inclusion_lemma}
	For every block with $\rho_i= 1$, for every $n\in \nats$, there exists $n'>n$ s.t. $\B_i^A(n)\subseteq\B_i(n')$.
	\end{lemma}
\begin{proof}[Proof sketch]
	%For the blocks with $\rho_i\neq 1$, this id obvious. Now, consider the case where $\rho_i=1$. 
	It is easy to see that given enough time, for every block of multiplicity $\sigma_i$ every point in the space $\reals^{\sigma_i}$ (or $\reals^{2\sigma_i}$) will eventually be covered by $\B_i$. One way to make that happen is to start from the very bottom element in each block and choose the corresponding controls $u_{\sigma_i}(\cdot)$ to reach the target in that coordinate. Then keep $u_{\sigma_i}(\cdot)=0$ and fix the dimension $i-1$ by choosing the right $u_{\sigma_{i-1}}(\cdot)$. Continuing this approach, one can show that $\B^{norm}_i$ can contain any point given enough space. (Since every control set will contain the origin, we can stop at any point.) This proves the statement of the lemma.
\end{proof}
Let $\T$ to be defined in the same sense as defined for the robust reachability problem ($\T = \operatorname{cl}(\{(\gamma_1^n,\ldots, \gamma_k^n) : n \in \nats\})$). Let $f:\nats \times \torus^k\to \reals^{D\times D}$ be the ``matrix builder'' function, defined as follows.
\[
f(n, (\alpha_1,\ldots, \alpha_k)) = \operatorname{diag}(g(\alpha_1),\ldots,g(\alpha_k), J_{k+1}^n, \ldots, J_{d}^n)
\] 
where
\[
g(\alpha_i) = \begin{bmatrix}
	A_i & n\Lambda_i^{-1}A_i & \cdots &\binom{n}{k-1}\Lambda_i^{\sigma_i+1}A_i\\
	& A_i & \ddots & \vdots\\
	&&\ddots n&  \Lambda_i^{-1}A_i\\
	&&&A_i 
\end{bmatrix}
\textrm{ and }
\MS{A_i = R(\alpha)}.
\]
Now, we can define the normalised abstraction as follows:
\[
\aepsilon(n)(z)= \MS{\bar D^n}f(n,z) x + \epsilon\B^A(n) \textrm{ and }  \aepsilon(n)=\{\aepsilon(n)(z) : z \in \T\},
\]
	%$$\aepsilon(n)=\bar D^n\T x+\epsilon \B^A(n),$$
	where $\bar D_i=\mathbb I$ (where $\mathbb I$ denotes the identity matrix of appropriate size) in every block except those ones with $\rho_i<1$. 
	 
	
	Now, consider the above abstraction. Lemmas 1, 2 (in the old version) should hold as o-minimality still holds. It remains to show that when Case~1 in Lemma~1 holds, we have pseudo-reachability. 
	\begin{lemma}
	Let Case~1 in Lemma~1 holds when $\varPhi(\epsilon,n)=\aepsilon(n)\cap S^{Proj}$. Then $S$ is pseudo-reachable.
	\end{lemma}
\begin{proof}
	%By Lemma~\ref{lem:inclusion_lemma}, we already know for every $$
	Let us fix $\epsilon>0$ and $\epsilon'$ such that $\epsilon'B\subseteq \frac{\epsilon}{4}\B(n)$ for all $n>0$. Then, there exists $p\in L(\epsilon/2)$ and for every $p^\ast$ satisfying $\|px-p^\ast x\|<\epsilon'/4$ (I notice that I'm a bit sloppy here and multiplication of $p$ and $p^\ast$ by the initial vector $x$; but, I think this is not a big issue and can be fixed.)
	such that $\mathcal{A}_{\epsilon/2}(n)(p^\ast)\cap S^{proj}\neq \emptyset$ for all $n>N$ ($N$ as defined in the proof of Lemma~3). Now, we select $N_2>N$ so that for all $n>N_2$, we have $\|M_i^nx\|<\epsilon'/8$ for all the blocks with $\rho_i<1$, where $M_i$ is the $i^{th}$ Jordan block in $M$. Now, we select $m, m'$ s.t. $m'>m>N_2$ and $\|R^mx-p^\ast x\|<\epsilon'$, $\|R^{m'}x-p^\ast x\|<\epsilon'$ and $\B^A(m)\subseteq \B(m')$. Similar to the argument made in the proof of Lemma~3, by additionally knowing that $\|\bar D_i^mR_i^m x\|<\epsilon'/2$ and $\|\bar D_i^{m'}R_i^{m'} x\|<\epsilon'/2$, we get that $\bar D^mp^\ast x\in R^{m'}x+\frac{\epsilon'}{4}B+\frac{\epsilon'}{4}B\subseteq \bar D^{m'}R^{m'}x+\frac{\epsilon}{2} \B(m)$ (note that $\bar D^i$ only scales down). This gives us that 
	$$\mathcal{A}_{\epsilon/2}(m)(p^\ast)=\bar D^mp^\ast x+\epsilon/2\B^A(m)\subseteq \bar D^{m'}R^{m'}x+\epsilon/2 \B(m')+\epsilon/2 \B(m')=\PO^{norm}_\epsilon(m').$$ This gives us what we wanted!
	\end{proof}
	

\begin{comment}
\section{Some questions}
\label{sec:questions}
Let us first fix one useful statement. Let $u_1,u_2,\dots$ to be n-dimensional vectors taken from the $l_2$ balls $\B_1,\B_2,\dots$, respectively, where the ball $\B_i$ is centered at the origin and has the radius $r_i$. More specifically, we can write $\|u_1\|\leq r_1$, $\|u_2\|\leq r_2$ and so on. Then, for $\alpha_i\geq 0$, we will have
\begin{align*}
	\|\sum_{i=1}^m \alpha_iu_i\|\leq \sum_{i=1}^m \alpha_i\|u_i\|\leq \sum_{i=1}^m \alpha_i r_i.
\end{align*}
Therefore, the sum of balls co-centered at the origin will be contained in a ball which is also centered at the origin and has the radius of size equal to sum of the radii for all the other balls.
\subsection{First: a simple one}
Consider the case where $M=\begin{bmatrix}1 &1\\0 &1\end{bmatrix}$, that is, $M$ is of Jordan real normal form and has one repeated (real) eigen value at $\lambda = 1$. Also let the bias term be absent ($b=\mathbf 0$). To my understanding, the proposed ``abstraction'' technique only affects the blocks with complex eigen values and all the rest of the blocks remain intact. In other words, $\PO_\epsilon(n)=\aepsilon(n)$ for all $n\in \nats$. Futher, we have $M^n=\begin{bmatrix}1 &n\\0 &1\end{bmatrix}$ and $\sum_{i=0}^{n-1}M^i=\begin{bmatrix}n &\frac{n(n+1)}{2}\\0 &n\end{bmatrix}$. Therefore, for a given initial state $s\in\reals^2$ and the control set $\B=[-1, 1]^2$, we have
$$
\B(n)=\begin{bmatrix}n &\frac{n(n+1)}{2}\\0 &n\end{bmatrix}\B=\begin{bmatrix}\frac{n(n+3)}{2}&0\\0 &n\end{bmatrix}\B,
$$
where the last equality holds because $M^i\geq 0$ (element-wise) for every $i\in  \nats$. Let $y(n)\in\PO_\epsilon(n)$. Then, for a given initial state $s=(s_1,s_2)$, we have $y(n)\in[s_1+n s_2-\epsilon\frac{n^2+3n}{2}, s_1+n s_2+\epsilon\frac{n^2+3n}{2}]\times[s_2-\epsilon n, s_2+\epsilon n]$. I think $\aepsilon(n)\cap S$ can be encoded as finite combination (conjunction and disjunction) of polynomials of $n$ and $\epsilon$ (using appropriate interval analysis). So, I don't understand why can't we answer the pseudo-reachability question for such $M$.
%I don't know how to encode the equality constraints in the target set $S\subset \reals^n$. But, for the strict inequalities, $\aepsilon(n)\cap S$ can be expressed in the form in Lemma,~\ref{lem::discrete-dichotomy}.  

\subsection{Second: maybe we can extend the results and answer decidability for the non-diagonalizable case(?)}
Let us consider the more general case where $M=\begin{bmatrix}\Lambda &I\\0 &\Lambda\end{bmatrix}$
and $\Lambda=\begin{bmatrix}\realpart(\lambda) &\im(\lambda)\\-\im(\lambda) &\realpart(\lambda)\end{bmatrix}$ with $\rho(\lambda)=1$. Also, we can use an abstraction technique similar to what we had and define
\[
\mathcal{T} = \operatorname{cl} \left( \{\Lambda^n : n \in \nats\} \right).
\]
Note that for $\B_i\subset \reals^2$, $i\in\{1,2\}$, we have $\mathcal{T}\B_i=\B_i$ (given for free because we selected the norm to be $l_2$). Now, we can again write 
$$
\B(n)=\begin{bmatrix}n\mathcal{T} &\frac{n(n+1)}{2}\mathcal{T}\\0 &n\mathcal{T}\end{bmatrix}\B=\begin{bmatrix}\frac{n(n+3)}{2}&0\\0 &n\end{bmatrix}\B.
$$
The above formulation seems to allow us for formulating decidability in non-diagonalizable case in FO logic. 
\end{comment}
